A Reciprocal Theorem for Finite Deformations in Incompressible Bodies

The reciprocal theorems of Maxwell and Betti are foundational in mechanics but have so far been restricted to infinitesimal deformations in elastic bodies. In this manuscript, we present a reciprocal theorem that relates solutions of a specific class of large deformation boundary value problems for incompressible bodies; these solutions are shown to identically satisfy the Maxwell-Betti theorem. The theorem has several potential applications such as development of alternative convenient experimental setups for the study of material failure through bulk and interfacial cavitation, and leveraging easier numerical implementation of equivalent auxiliary boundary value problems. The following salient features of the theorem are noted: (i) it applies to dynamics in addition to statics, (ii) it allows for large deformations, (iii) generic body shapes with several potential holes, and (iv) any general type of boundary conditions.

==> Reciprocal theorem JMPS submit_Arxiv/settings.tex <==

\usepackage{amsmath}
\newcommand\abs[1]{\left|#1\right|}
\usepackage{amssymb}
\usepackage{subfiles} %permet d'avoir des sous fichiers
\usepackage{subcaption}
\usepackage{multicol}
\usepackage{bm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Graphics
\usepackage{graphicx}
%\usepackage[font=footnotesize]{subfig}
\usepackage[export]{adjustbox}
\usepackage[font=footnotesize]{caption}
\usepackage{float} %picture placement
\usepackage{placeins}%floatbarrier
    \floatplacement{figure}{h}
    \floatplacement{table}{h}
\usepackage[dvipsnames]{xcolor}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\definecolor{red}{rgb}{1,0,0}
\definecolor{black}{rgb}{0,0,0}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.65,0,0.82}
\definecolor{backcolour}{rgb}{0.97,0.97,0.97}
\definecolor{codeorange}{rgb}{1,0.31,0}
\usepackage{longtable}
\renewcommand{\arraystretch}{1.4} %jolie tableau

%OTHERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{xparse}
        \ExplSyntaxOn
        \NewDocumentCommand{\convertto}{mm}
                % #1 = em or ex (or any other unit)
                % #2 = dimen to convert
         {  \texttt{#2~=~\fp_to_decimal:n { (#2)/(1#1) }#1} }
         \ExplSyntaxOff
\newcommand{\image}[2][]{%
    \includegraphics[height=5cm]{#2}}
\newcommand{\twoimage}[2][]{%
    \includegraphics[width=0.48\textwidth]{#2}}
\newcommand{\grad}{\nabla}   
\def\R{\textsuperscript{\textregistered}}
\def\tcf{\centering\footnotesize}

\usepackage[per-mode=symbol]{siunitx}

%\newcommand\unit[1]{~[\si{#1}]~}
\newcommand{\bbbox}[1]{\setlength{\fboxsep}{0pt}
\setlength{\fboxrule}{0.8pt}\fbox{#1}}
\newcommand\ssfrac[2]{#1/#2}
\newcommand{\ta}{\large{$a$ }\normalsize }

